S2AMP: A High-Coverage Dataset of Scholarly Mentorship Inferred from Publications

Mentorship is a critical component of academia, but is not as visible as publications, citations, grants, and awards. Despite the importance of studying the quality and impact of mentorship, there are few large representative mentorship datasets available. We contribute two datasets to the study of mentorship. The first has over 300,000 ground truth academic mentor-mentee pairs obtained from multiple diverse, manually-curated sources, and linked to the Semantic Scholar (S2) knowledge graph. We use this dataset to train an accurate classifier for predicting mentorship relations from bibliographic features, achieving a held-out area under the ROC curve of 0.96. Our second dataset is formed by applying the classifier to the complete co-authorship graph of S2. The result is an inferred graph with 137 million weighted mentorship edges among 24 million nodes. We release this first-of-its-kind dataset to the community to help accelerate the study of scholarly mentorship: \url{https://github.com/allenai/S2AMP-data}

==> sections/related_work.tex <==
% -  This can be in two parts:

% \begin{itemize}
%     \item Modelling related work : what techniques and datasets were used previously and what worked and why our approach might be better
    
    
% \begin{itemize}
%     \item \cite{Lee2020} Web of scholars: very relevant work, 1 million authors in MAG are predicted with advisors using Shifu2 [R3]
%     \item \cite{Liu2020} Node and edge attributes are used to train a classifier on collaboration network [R3]
%     \item \cite{Wang1145} Poster paper for first version of Shifu [R3]
%     \item \cite{Rao2010} models the advisor-advisee relationship mining problem using a jointly likelihood objective function. Most papers here cites this paper [R3]
%     \item \cite{Jean11723} Graphical properties of the mentorship network and semantic properties of mentor and trainee publications are used for analysis [R1]
%     \item \cite{tang2011learning} Advisor-advisee prediction is one of the tasks on which their model is trained on  [R2]
%     \item \cite{Tao2013} prediction of Advisor-Advisee Relationship and Historical Affiliations [R1] 
    
% \end{itemize}
    
%     \item Science of science related work : what predictions or studies were done by previous work
    
%     \begin{itemize}
%     \item \cite{AlShebli2020} Makes multiple assumptions (strict threshold of 7 years, predicting gender with first name) which led to flawed findings
%     Dataset: MAG
%     Key questions:
%     Model: 
%     Disambiguation: Use rules \footnote{\url{https://static-content.springer.com/esm/art\%3A10.1038\%2Fs41467-020-19723-8/MediaObjects/41467_2020_19723_MOESM1_ESM.pdf}}
% \item \cite{Yifang1073}  Mentorship is associated with a 2X to 4X rise in a protégé's likelihood of prizewinning,
% \item \cite{Malmgren2010} 
% \begin{itemize}
%     \item Questions: number of mentees mentored is correlated with other measures of academic success
%     \item Data: Mathematics Genealogy Project
% \end{itemize}
% \item \cite{Schwartz2021} 
% \begin{itemize}
%     \item Questions: Analysis on gender done by academic tree people. Trainees of female mentors are less likely to continue into independent research careers than trainees of male mentors. 
%     \item Data: Academic tree
% \end{itemize}
% \item \cite{Sinatra2016} 
% \begin{itemize}
%     \item Questions: study of temporal career patterns that characterize the emergence of scientific excellence
%     \item Data: Physical Review data set - http://journals.aps.org/datasets, combination of 24,630 Google Scholar career profiles with Web of Science (WoS) data
% \end{itemize}
% \item \cite{Linard2018IntellectualSI}
% \begin{itemize}
%     \item Questions: successful mentors tend to train successful students. But what characteristics of this relationship predict success, and how? Researchers were more likely to succeed if they trained under mentors with disparate expertise and integrated that expertise into their own work.
%     \item Data: Academic Family Tree
% \end{itemize}
% \item \cite{Sugimoto2011AcademicGA}
% \begin{itemize}
%     \item Questions: Proposes use of academic genealogy as an indicator of interdisciplinarity and calls for additional research on the role of doctoral committee composition in a student’s subsequent academic career.
%     \item Data: 3,038 PhD dissertations in Library and Information Science (LIS)
% \end{itemize}
% \item \cite{Sekara2018TheCE}
% \begin{itemize}
%     \item Questions: Develop a quantitative understanding of author order by quantifying this “chaperone effect,” capturing how scientists transition into senior status within a particular publication venue.
%     \item Data:  publication data provided by the Web of Science 
% \end{itemize}
% \item \cite{Petersen2015QuantifyingTI}
% \begin{itemize}
%     \item Questions: analyze the collaboration network from a researcher’s local perspective along his/her career. Their approach reveals that scientific collaboration is characterized by a high turnover rate juxtaposed with surprisingly frequent "life partners." 
%     \item Data: Thompson Reuters Web of Knowledge (TRWOK)
% \end{itemize}
% \item \cite{Li2019EarlyCW}
% \begin{itemize}
%     \item Questions: Examined the long-term impact of coauthorship with established, highly-cited scientists on the careers of junior researchers in four scientific disciplines. Early coauthorship predicts a higher probability of repeatedly coauthoring work with top-cited scientists, and, ultimately,a higher probability of becoming one.
%     \item Data: Web of Science database
% \end{itemize}
% \item \cite{Rossi2017GenealogicalIA}
% \begin{itemize}
%     \item Questions: We show that Ph.D. students benefit from having multiple supervisors instead of a single one. The cognitive diversity of mentors has a subtler effect in that it increases both the likelihood of success (having many mentees later on) and failure (having no mentees at all later on).
%     \item Data: Math genealogy
% \end{itemize}
% \item \cite{Chariker2017IdentificationOS}
% \begin{itemize}
%     \item Questions: Do Nobel Laureates cluster in mentorship lineages?
%     \item Data: Academic Family Tree
% \end{itemize}
% \item \cite{Way2019ProductivityPA}
% \begin{itemize}
%     \item Questions: We find that faculty’s work environments, not selection effects, drive their productivity and prominence, establishing that where a researcher works serves as a mechanism for cumulative advantage, locking in past success via job placement and thereby facilitating future success.
%     \item Data: We reconstruct these experiments from a unique and comprehensive dataset that documents the doctorate-to-faculty transitions of 2,453 tenuretrack faculty at all 205 PhD-granting computer science departments in the United States and Canada, spanning 1970–2011, along with complete records of their scholarly output through 2017, encompassing more than 200,000 publications and 7.4 million citations.
% \end{itemize}
% \item \cite{Dores2016ExtractingAG}
% \begin{itemize}
%     \item Questions: Not much, looks at "width" vs "depth" of an academic's tree
%     \item Data: Networked Digital Library of Theses and Dissertations
% \end{itemize}
% \item \cite{Heinisch2018TheNG}
% \begin{itemize}
%     \item Questions: Can we we predict advisor-advisee relationships? How do various things impact the likelihood of a mentee to become mentor?
%     \item Data: German physics PhD data
% \end{itemize}
% \item \cite{Sanyal2020gmindexAN}
% \begin{itemize}
%     \item Questions: Can we create an h-index but for mentorship?
%     \item Data: Mathematics Genealogy Project and the Academic Family Tree
% \end{itemize}
% \end{itemize}
    
    
%   Datasets : \cite{Ke2021} Academic Tree dataset linked with MAG - 490k authors [R3]
% \end{itemize}

